Competence-Aware Path Planning via Introspective Perception

Robots deployed in the real world over extended periods of time need to reason about unexpected failures, learn to predict them, and to proactively take actions to avoid future failures. Existing approaches for competence-aware planning are either model-based, requiring explicit enumeration of known failure modes, or purely statistical, using state- and location-specific failure statistics to infer competence. We instead propose a structured model-free approach to competence-aware planning by reasoning about plan execution failures due to errors in perception, without requiring a priori enumeration of failure sources or requiring location-specific failure statistics. We introduce competence-aware path planning via introspective perception (CPIP), a Bayesian framework to iteratively learn and exploit task-level competence in novel deployment environments. CPIP factorizes the competence-aware planning problem into two components. First, perception errors are learned in a model-free and location-agnostic setting via introspective perception prior to deployment in novel environments. Second, during actual deployments, the prediction of task-level failures is learned in a context-aware setting. Experiments in a simulation show that the proposed CPIP approach outperforms the frequentist baseline in multiple mobile robot tasks, and is further validated via real robot experiments in an environment with perceptually challenging obstacles and terrain.

==> acknowledgments.tex <==
\section{Acknowledgments}
This work is supported in part by NSF (CAREER-2046955,
IIS-1954778) and DARPA (HR001120C0031). The views and conclusions contained in this document are
those of the authors only.

==> background.tex <==



==> planning_background.tex <==
\section{Planning Model Description} \label{sec:planning_background}
The input to our problem is a topological map of the environment in the form of a directed graph $G$ composed of a set of nodes, $N$, and a set of edges, $E \subseteq N^2$. Each nodes represents a location (i.e. an $xy$--coordinate), and each edge $e$ is associated with a corresponding value $t_e$, denoting the expected traversal time for the edge, and $p_e$, denoting the probability of successfully traversing the edge.

Given the topological map, $G$, we model the planning problem as a Stochastic Shortest Path (SSP) problem, a formal decision-making model for reasoning in stochastic environments where the objective is to find the least-cost path from a start state to a goal state. An SSP is a tuple $\langle S, A, T, C, s_0, G \rangle$ where $S$ is a finite set of states, $A$ is a finite set of actions, $T : S \times A \times S \rightarrow [0,1]$ represents the probability of reaching state $s' \in S$ after performing action $a \in A$ in state $s \in S$, $C : S \times A \rightarrow \mathbb{R}^+$ represents the expected immediate cost of performing action $a \in A$ in state $s \in S$, $s_0 \in S$ is an initial state, and $G \subset S$ is a finite (possibly singleton) set of goal states such that $T(s_g, a, s_g) = 1 \land C(s_g, a) = 0 \hspace{1mm} \forall a \in A, s_g \in G$.

A solution to an SSP is a policy $\pi : S \rightarrow A$ that indicates that action $\pi(s) \in A$ should be taken in state $s \in S$. A policy $\pi$ induces the value function $V^{\pi} : S \rightarrow \mathbb{R}$ that represents the expected cumulative cost $V^{\pi}(s)$ of reaching $s_g$ from state $s$ following the policy $\pi$. An optimal policy $\pi^*$ minimizes the expected cumulative cost $V^*(s_0)$ from the initial state $s_0$.

In our problem, $S = N \times \tilde{S}$ is a finite set of states comprised of the map nodes $N$ and a finite set of failure states $\tilde{S}$ and $A = E \cup \tilde{A}$ is a finite set of actions comprised of the directed edges in the graph and a finite set of recovery actions $\tilde{A}$. $T(s,a,s')$ is determined by the probability of successfully traversing the edge $e = (s,s')$, $p_e$, which is zero if the action $a$ does not correspond to the edge $e$, and whether the current state is a failure state. In a failure state $s$, $T(s, a, s') = 0$ if $a \notin \tilde{A}$ and $s \neq s'$. $C(s,a)$ is set to $t_e$ if $a \in E$, and the expected recovery cost for $s$ otherwise.





